Multi-Modal Adapter for Vision-Language Models

Large pre-trained vision-language models, such as CLIP, have demonstrated state-of-the-art performance across a wide range of image classification tasks, without requiring retraining. Few-shot CLIP is competitive with existing specialized architectures that were trained on the downstream tasks. Recent research demonstrates that the performance of CLIP can be further improved using lightweight adaptation approaches. However, previous methods adapt different modalities of the CLIP model individually, ignoring the interactions and relationships between visual and textual representations. In this work, we propose Multi-Modal Adapter, an approach for Multi-Modal adaptation of CLIP. Specifically, we add a trainable Multi-Head Attention layer that combines text and image features to produce an additive adaptation of both. Multi-Modal Adapter demonstrates improved generalizability, based on its performance on unseen classes compared to existing adaptation methods. We perform additional ablations and investigations to validate and interpret the proposed approach.

==> sections/0_abstract.tex <==
Large pre-trained vision-language models, such as CLIP \cite{radford2021learning}, have demonstrated state-of-the-art performance across a wide range of image classification tasks, without requiring retraining. Few-shot CLIP is competitive with existing specialized architectures that were trained on the downstream tasks. Recent research demonstrates that the performance of CLIP can be further improved using lightweight adaptation approaches. 
However, previous methods adapt different modalities of the CLIP model individually, ignoring the interactions and relationships between visual and textual representations.
In this work, we propose Multi-Modal Adapter, an approach for Multi-Modal adaptation of CLIP. Specifically, we add a trainable Multi-Head Attention layer that combines text and image features to produce an additive adaptation of both. Multi-Modal Adapter demonstrates improved generalizability, based on its performance on unseen classes compared to existing adaptation methods. We perform additional ablations and investigations to validate and interpret the proposed approach.

==> sections/x_guidelines.tex <==
\section*{Submission Policy}

Paper submission should be solely done over Canvas. The guidelines below will be enforced for the paper:
\begin{itemize}
\item Submissions must be in PDF\@. 
\item If your paper has appendices, submit the appendix together with the main body and the references \textbf{as a single file}.
\item Page limit: The main body of the paper has to be fitted to \textbf{8 pages}, excluding references and appendices; the space for the latter two is not limited.
\item Your paper should be in \textbf{10 point Times font}.
\item Make sure your PDF file only uses Type-1 fonts.
\item Place figure captions \emph{under} the figure (and omit titles from inside the graphic file itself). Place table captions \emph{over} the table.
\item References must be in author-year format, as shown in the default style file. Example: in-place \citet{brown2020language}, after-sentence \cite{brown2020language}. Multiple citations should be placed in chronological order, e.g. \cite{brown2020language, dosovitskiy2020image}.
\item Do not alter the style template; in particular, do not compress the paper format by reducing the vertical spaces.
\item Keep your abstract brief and self-contained, one paragraph and roughly 4--6 sentences. 
\item The title should have content words capitalized.
\end{itemize}
This section \textit{Submission Policy} should not be included in the final paper.
